LP++: A Surprisingly Strong Linear Probe for Few-Shot CLIP

In a recent, strongly emergent literature on few-shot CLIP adaptation, Linear Probe (LP) has been often reported as a weak baseline. This has motivated intensive research building convoluted prompt learning or feature adaptation strategies. In this work, we propose and examine from convex-optimization perspectives a generalization of the standard LP baseline, in which the linear classifier weights are learnable functions of the text embedding, with class-wise multipliers blending image and text knowledge. As our objective function depends on two types of variables, i.e., the class visual prototypes and the learnable blending parameters, we propose a computationally efficient block coordinate Majorize-Minimize (MM) descent algorithm. In our full-batch MM optimizer, which we coin LP++, step sizes are implicit, unlike standard gradient descent practices where learning rates are intensively searched over validation sets. By examining the mathematical properties of our loss (e.g., Lipschitz gradient continuity), we build majorizing functions yielding data-driven learning rates and derive approximations of the loss's minima, which provide data-informed initialization of the variables. Our image-language objective function, along with these non-trivial optimization insights and ingredients, yields, surprisingly, highly competitive few-shot CLIP performances. Furthermore, LP++ operates in black-box, relaxes intensive validation searches for the optimization hyper-parameters, and runs orders-of-magnitudes faster than state-of-the-art few-shot CLIP adaptation methods. Our code is available at: \url{https://github.com/FereshteShakeri/FewShot-CLIP-Strong-Baseline.git}.

==> sec/Additional-results.tex <==
% \section{Ablation Study}
% \textbf{Comparison of adapter methods based on number of parameters}

% \begin{table}[h]
% \footnotesize
% \setlength{\tabcolsep}{3pt}
% \centering
% \begin{tabular}{lccc}
% \toprule
%  Methods & \#Parameters & Exp(S=16,K=1000) & Exp(S=16,K=101) \\
% \midrule
% \midrule

% %\textit{CLIP-based Adapters} & & \\
% %\hdashline
%  Clip-Adapter\cite{Gao2023clipadapter} & $2 (D_1 \times D_2)$ &  $\sim525k$ & $\sim525k$\\
% Tip-adapter-F\cite{zhang2022tip} & $K \times S \times D$ & $\sim16m$ & $\sim1.6m$\\
% \midrule
% LP++  & $K (D + 1)$ & $\sim1m$ & $\sim103k$ \\
% \bottomrule
% \end{tabular}
% \caption{Comparison of adapter methods and LP++ based on number of parameters. The last two columns are calculated for datasets with 1000 (e.g. ImagenNet) and 101 (e.g. Caltech101) classes in the 16 shot setting. In the above table, $D_1=256$, and $D_2 = D = 1024$. }
% \label{table:time_Imagenet}
% \end{table}

\begin{figure*}
     \centering

     \includegraphics[width=0.9\linewidth]{figures/main-fig2.pdf}

    \caption{Comparison of LP++ with different adaptation methods on 9 benchmarks, which are averaged over 10 tasks.}
    \label{fig:main2-sup}
\end{figure*}

\section{Ranking}
 In Fig.~\ref{fig:autorank}, we show the ranking of different methods using Autorank\cite{Herbold2020} (on the 11 datasets); lower value indicates better performance.
 
\begin{figure}
\centering
\includegraphics[width=0.8\linewidth]{figures/autorank.pdf}
\caption{Comparison of ranking of different methods using Autorank\cite{Herbold2020}. The results are averaged over 11 datasets.}
\label{fig:autorank}
\end{figure}

\section{Additional numerical results on 11 benchmarks}
\label{sec:additional_results}
~\cref{table:resultOther_AllDatasets_details} shows the average accuracy and standard deviation over 10 tasks for LP++ and the baseline methods on 11 benchmarks. The per-dataset performance across all the methods and for different number of shots %averaged over 10 tasks 
is depicted in ~\cref{fig:main2-sup}, which complements \cref{fig:clip_mag} in the main paper. In these plots, we can observe that LP++ (\textit{green curve}) yields the best overall performance in 6 out of 11 data sets. Furthermore, LP++ outperforms all adapter-based methods in nearly all remaining datasets and scenarios (i.e., varying number of shots). Only in a few cases, e.g., FGVCAirCraft and OxfordPets, Tip-Adapter-F* provides better performance than our proposed approach. Indeed, the largest improvement gains are observed in FGVCAirCraft, where the accuracy obtained by all methods is considerably small. We believe that, in this particular scenario, the more intensive grid search carried out by Tip-Adapter-F* has a greater impact on its results. Considering %Regarding the results obtained by 
prompt learning strategies, ProGrad is the highest performing approach, which obtains the best overall results in several datasets. Nevertheless, in addition to the limitations already highlighted for these methods (i.e., time complexity and non-suitability for black-box adaptation), the large standard deviation observed across runs (see also \cref{fig:avg-std}), makes these approaches highly unreliable, specially in the low-labeled data regime. As discussed, this could be due to the fact that these approaches learn prompts, through the text encoder, which are %might be 
``too specialized'' for a given image support set.

\begin{table*}[ht] 
\footnotesize
\tiny
\centering
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{l|lccccc}
\hline
 Dataset & \textbf{Number of shots ($S$)} & \textbf{1} & \textbf{2} & \textbf{4} & \textbf{8} & \textbf{16}\\
\hline
\hline
\multirow{10}{*}{\textit{ImageNet}} & Zero-shot CLIP$_\text{ ICML'21}$\cite{radford2021clip} & \multicolumn{5}{c}{60.35}\\
\cline{2-7}
& CoOp$_\text{ IJCV'22}$\cite{Zhou2022coop} & $61.19 \pm 0.17$ & $61.58 \pm 0.40$  &  $62.22 \pm 0.22$  & $62.87 \pm 0.21$  &  $63.70 \pm 0.13$ \\
& PLOT$_\text{ ICLR'23}$\cite{chen2023plot} & $60.46 \pm 0.34$ &  $60.73 \pm 0.60$ &  $61.79 \pm 0.39$  &  $62.48 \pm 0.32$ & $63.08 \pm 0.26$  \\
& KgCoOp$_\text{ CVPR'23}$\cite{Yao2023kgcoop} & $60.90 \pm 0.16$ & $61.44 \pm 0.15$ & $62.00 \pm 0.11$ &$62.20 \pm 0.15$ & $62.43 \pm 0.11$ \\
& ProGrad$_\text{ ICCV'23}$\cite{Zhu2023prograd} & $\bm{61.58} \pm 0.27$ & $\bm{62.14} \pm 0.13$ & $\bm{62.59} \pm 0.09$ & $63.04 \pm 0.11$ & $63.54 \pm 0.18$\\
\cline{2-7}
%Tip-Adapter\cite{zhang2022tip} & $60.48\pm0.08$ & $60.56\pm0.16$ & $61.02\pm0.12$ & $61.24\pm0.08$ & $61.59\pm0.10$ \\
%\hline
& CLIP-Adapter$_\text{ IJCV'23}$\cite{Gao2023clipadapter} & $59.82 \pm 0.11 $ & $59.94 \pm 0.05$ & $59.97 \pm 0.04$ & $59.98 \pm 0.09$ & $ 61.31 \pm 0.39$ \\
& Tip-Adapter-F$_\text{ ECCV'22}$\cite{zhang2022tip} & $60.59 \pm0.14$ & $61.42 \pm0.05$ & $62.12 \pm0.06$  & $63.41\pm 0.07$  & $\bm{65.06}\pm 0.04$ \\
& Tip-Adapter-F*$_\text{ ECCV'22}$\cite{zhang2022tip} & $60.98 \pm0.15$ & $61.23 \pm0.11$ & $61.72 \pm0.25$ & $62.84\pm 0.10$ & $64.03\pm 0.12$ \\
%\textcolor{blue}{(-0.48)}
\cline{2-7}
& Standard LP$_\text{ ICML'21}$\cite{radford2021clip} & $22.21 \pm 0.31$  &  $31.96 \pm0.25$  &  $41.48 \pm0.25$  &  $49.49 \pm0.16$  & $56.04 \pm0.13$  \\
& \cellcolor{blue!15}{LP++} & \cellcolor{blue!15}{$61.18 \pm 0.08$} &  \cellcolor{blue!15}{$61.56 \pm 0.14$} & \cellcolor{blue!15}{$62.55 \pm 0.12$} & \cellcolor{blue!15}{$\bm{63.76} \pm 0.07$} & \cellcolor{blue!15}{$64.73 \pm  0.05$}\\
\midrule

\multirow{10}{*}{\textit{SUN397}} & Zero-shot CLIP$_\text{ ICML'21}$\cite{radford2021clip} & \multicolumn{5}{c}{58.85}\\
\cline{2-7}
& CoOp$_\text{ IJCV'22}$\cite{Zhou2022coop} &$61.79 \pm 0.45$ &  $63.32 \pm 0.47$ & $65.79 \pm 0.44$ & $67.89 \pm 0.38$  &  $70.15 \pm 0.32$ \\
& PLOT$_\text{ ICLR'23}$\cite{chen2023plot} & $62.53 \pm 0.30$ & $63.87 \pm 0.26$ & $65.85 \pm 0.48$ & $67.83 \pm 0.36$ & $69.90 \pm 0.31$  \\
& KgCoOp$_\text{ CVPR'23}$\cite{Yao2023kgcoop} & $\bm{62.91} \pm 0.59$  &  $64.38 \pm 0.30$ & $66.06 \pm 0.37$ & $66.66 \pm 1.10$ & $67.68 \pm 0.78$ \\
& ProGrad$_\text{ ICCV'23}$\cite{Zhu2023prograd} & $62.79 \pm 0.50$ & $64.12 \pm 0.55$ & $66.32 \pm 0.59$ & $68.33 \pm 0.28$ & $70.18 \pm 0.27$\\
\cline{2-7}
%Tip-Adapter\cite{zhang2022tip} & $60.48\pm0.08$ & $60.56\pm0.16$ & $61.02\pm0.12$ & $61.24\pm0.08$ & $61.59\pm0.10$ \\
%\hline
& CLIP-Adapter$_\text{ IJCV'23}$\cite{Gao2023clipadapter} & $60.78 \pm 0.16 $ & $61.79 \pm 0.23$ & $63.84 \pm 0.35$ & $66.26 \pm 0.14$ & $ 67.66 \pm 1.05$ \\
& Tip-Adapter-F$_\text{ ECCV'22}$\cite{zhang2022tip} & $61.02 \pm 0.36$  & $62.15 \pm 0.28$  & $63.86 \pm 0.19$ & $67.25 \pm 0.16$ & $70.94 \pm 0.13$ \\
& Tip-Adapter-F*$_\text{ ECCV'22}$\cite{zhang2022tip} & $62.58 \pm 0.22$  & $63.79 \pm 0.13$  & $65.49 \pm 0.35$ & $67.43 \pm 0.11$ & $69.25 \pm 0.16$ \\
%\textcolor{blue}{(-0.48)}
\cline{2-7}
& Standard LP$_\text{ ICML'21}$\cite{radford2021clip} & $32.56 \pm 0.40$  & $43.77 \pm 0.41$   &  $54.49 \pm 0.39$  &  $61.83 \pm 0.30$  &  $67.03 \pm 0.16$  \\
& \cellcolor{blue!15}{LP++} & \cellcolor{blue!15}{$62.47 \pm 0.27$} & \cellcolor{blue!15}{$\bm{64.65} \pm 0.25$} & \cellcolor{blue!15}{$\bm{67.28} \pm 0.27$} & \cellcolor{blue!15}{$\bm{69.34} \pm 0.14$} & \cellcolor{blue!15}{$\bm{71.23} \pm 0.07$}\\
\midrule

\multirow{10}{*}{\textit{DTD}} & Zero-shot CLIP$_\text{ ICML'21}$\cite{radford2021clip} & \multicolumn{5}{c}{42.69}\\
\cline{2-7}
& CoOp$_\text{ IJCV'22}$\cite{Zhou2022coop} & $42.31 \pm 1.86$ &  $47.13 \pm 1.93$ &  $54.06 \pm 1.49$  & $59.21 \pm 0.91$  &  $63.67 \pm 0.83$ \\
& PLOT$_\text{ ICLR'23}$\cite{chen2023plot} & $45.82 \pm 1.72$ & $51.32 \pm 1.61$  & $55.67 \pm 1.14$   &  $61.38 \pm 1.04$ &  $65.29 \pm 1.05$  \\
& KgCoOp$_\text{ CVPR'23}$\cite{Yao2023kgcoop} & $45.46 \pm 2.83$ & $50.01 \pm 2.71$ & $53.37 \pm 0.71$ &  $58.38 \pm 1.34$  & $62.71 \pm 0.92$ \\
& ProGrad$_\text{ ICCV'23}$\cite{Zhu2023prograd} & $44.19 \pm 2.38$  & $ 50.41 \pm 1.74$  & $54.82 \pm 1.28$ & $60.31 \pm 0.99$ & $63.89 \pm 0.88$\\
\cline{2-7}
%Tip-Adapter\cite{zhang2022tip} & $60.48\pm0.08$ & $60.56\pm0.16$ & $61.02\pm0.12$ & $61.24\pm0.08$ & $61.59\pm0.10$ \\
%\hline
& CLIP-Adapter$_\text{ IJCV'23}$\cite{Gao2023clipadapter} & $43.49 \pm 0.68 $ & $44.49 \pm 1.07$ & $48.95 \pm 0.85$ & $57.52 \pm 0.67$ & $ 62.97 \pm 0.60$ \\
& Tip-Adapter-F$_\text{ ECCV'22}$\cite{zhang2022tip} & $46.92 \pm 1.01$ & $48.50 \pm 1.08$ & $57.16 \pm 0.53$ & $62.38 \pm 0.47$ & $65.23 \pm 0.82$ \\
& Tip-Adapter-F*$_\text{ ECCV'22}$\cite{zhang2022tip} & $\bm{47.68} \pm 1.43$ & $52.24 \pm 0.74$ & $56.09 \pm 0.99$ & $61.05 \pm 0.71$ & $65.04 \pm 0.21$ \\
%\textcolor{blue}{(-0.48)}
\cline{2-7}
& Standard LP$_\text{ ICML'21}$\cite{radford2021clip} & $29.63 \pm 1.53$ & $41.19 \pm 1.45$   & $51.72 \pm 0.57$   &  $58.78 \pm 0.52$  & $64.56 \pm 0.69$  \\
& \cellcolor{blue!15}{LP++} & \cellcolor{blue!15}{$46.97 \pm 1.37$} & \cellcolor{blue!15}{$\bm{52.44} \pm 0.99$} & \cellcolor{blue!15}{$\bm{57.75} \pm 0.82$} & \cellcolor{blue!15}{$\bm{62.42} \pm 0.53$} & \cellcolor{blue!15}{$\bm{66.40} \pm 0.50$}\\
\midrule

\multirow{10}{*}{\textit{Caltech101}} & Zero-shot CLIP$_\text{ ICML'21}$\cite{radford2021clip} & \multicolumn{5}{c}{85.84}\\
\cline{2-7}
& CoOp$_\text{ IJCV'22}$\cite{Zhou2022coop} & $87.06 \pm 1.24$ & $89.14 \pm 0.87$  &  $90.00 \pm 0.63$  &  $91.00 \pm 0.66$ &  $91.77 \pm 0.29$ \\
& PLOT$_\text{ ICLR'23}$\cite{chen2023plot} & $\bm{89.41} \pm 0.41$ & $\bm{90.22} \pm 0.25$  &  $90.69 \pm 0.37$  &  $91.55 \pm 0.38$ &  $92.17 \pm 0.30$  \\
& KgCoOp$_\text{ CVPR'23}$\cite{Yao2023kgcoop} & $88.24 \pm 0.49$ & $88.85 \pm 0.43$  &  $89.89 \pm 0.31$ & $90.32 \pm 0.43$ & $90.93 \pm 0.26$ \\
& ProGrad$_\text{ ICCV'23}$\cite{Zhu2023prograd} & $88.34 \pm 1.64$  & $89.01 \pm 0.61$  & $90.13 \pm 0.45$  & $90.76 \pm 0.32$ & $91.67 \pm 0.39$\\
\cline{2-7}
%Tip-Adapter\cite{zhang2022tip} & $60.48\pm0.08$ & $60.56\pm0.16$ & $61.02\pm0.12$ & $61.24\pm0.08$ & $61.59\pm0.10$ \\
%\hline
& CLIP-Adapter$_\text{ IJCV'23}$\cite{Gao2023clipadapter} & $87.69 \pm 0.41 $ & $89.37 \pm 0.29$ & $90.21 \pm 0.32$ & $91.33 \pm 0.15$ & $ 92.10 \pm 0.20$ \\
& Tip-Adapter-F$_\text{ ECCV'22}$\cite{zhang2022tip} & $87.35 \pm 0.64$ & $88.17 \pm 0.29$ & $89.49 \pm 0.25$ & $90.54 \pm 0.34$ & $92.10 \pm 0.25$ \\
& Tip-Adapter-F*$_\text{ ECCV'22}$\cite{zhang2022tip} & $88.68 \pm 0.44$ & $89.36 \pm 0.59$ & $90.40 \pm 0.26$ & $91.62 \pm 0.23$ & $92.63 \pm 0.21$ \\
%\textcolor{blue}{(-0.48)}
\cline{2-7}
& Standard LP$_\text{ ICML'21}$\cite{radford2021clip} & $68.88 \pm 1.68$  &  $78.41 \pm 0.54$  &  $84.91 \pm 0.45$  &  $88.70 \pm 0.40$  &  $91.14 \pm 0.19$  \\
& \cellcolor{blue!15}{LP++} & \cellcolor{blue!15}{$88.56 \pm 0.43$} & \cellcolor{blue!15}{$89.53 \pm 0.35$} & \cellcolor{blue!15}{$\bm{90.87} \pm 0.19$} & \cellcolor{blue!15}{$\bm{91.84} \pm 0.24$} & \cellcolor{blue!15}{$\bm{92.73} \pm 0.17$}\\
\midrule

\multirow{10}{*}{\textit{UCF101}} & Zero-shot CLIP$_\text{ ICML'21}$\cite{radford2021clip} & \multicolumn{5}{c}{61.80}\\
\cline{2-7}
& CoOp$_\text{ IJCV'22}$\cite{Zhou2022coop} & $62.80 \pm 1.26$ &  $65.62 \pm 1.09$ & $68.69 \pm 0.76$  &  $72.57 \pm 0.80$ & $76.39 \pm 0.54$ \\
& PLOT$_\text{ ICLR'23}$\cite{chen2023plot} & $63.22 \pm 1.05$ & $66.49 \pm 0.92$& $70.12 \pm 0.62$& $74.63 \pm 0.79$ & $77.39 \pm 0.53$  \\
& KgCoOp$_\text{ CVPR'23}$\cite{Yao2023kgcoop} & $64.37 \pm 1.66$  & $64.91 \pm 1.01$ & $68.41 \pm 0.38$  & $69.86 \pm 0.33$ &  $71.73 \pm 0.78$ \\
& ProGrad$_\text{ ICCV'23}$\cite{Zhu2023prograd} & $65.13 \pm 0.87$  & $66.57 \pm 0.62$ & $69.80 \pm 0.62$ & $73.01 \pm 0.52$ & $75.76 \pm 0.47$\\
\cline{2-7}
%Tip-Adapter\cite{zhang2022tip} & $60.48\pm0.08$ & $60.56\pm0.16$ & $61.02\pm0.12$ & $61.24\pm0.08$ & $61.59\pm0.10$ \\
%\hline
& CLIP-Adapter$_\text{ IJCV'23}$\cite{Gao2023clipadapter} & $64.25 \pm 0.54 $ & $66.68 \pm 0.31$ & $69.77 \pm 0.40$ & $73.90 \pm 0.50$ & $ 77.26 \pm 0.39$ \\
& Tip-Adapter-F$_\text{ ECCV'22}$\cite{zhang2022tip} & $64.28 \pm 0.54$ & $65.48 \pm 0.43$ & $67.61 \pm 0.28$ & $72.05 \pm 0.53$ & $77.30 \pm 0.21$  \\
& Tip-Adapter-F*$_\text{ ECCV'22}$\cite{zhang2022tip} & $\bm{65.50} \pm 0.59$ & $68.55 \pm 0.45$ & $70.55 \pm 0.58$ & $74.25 \pm 0.48$ & $76.83 \pm 0.24$  \\
%\textcolor{blue}{(-0.48)}
\cline{2-7}
& Standard LP$_\text{ ICML'21}$\cite{radford2021clip} & $40.80 \pm 1.05$ &  $51.71 \pm 0.79$  &  $61.64 \pm 0.50$  &  $68.47 \pm 0.44$  &  $73.38 \pm 0.43$  \\
& \cellcolor{blue!15}{LP++} & \cellcolor{blue!15}{$65.41 \pm 0.37$} & \cellcolor{blue!15}{$\bm{69.20} \pm 0.52$} & \cellcolor{blue!15}{$\bm{71.68} \pm 0.41$} & \cellcolor{blue!15}{$\bm{74.86} \pm 0.36$} & \cellcolor{blue!15}{$\bm{77.46} \pm 0.39$}\\
\midrule

\multirow{10}{*}{\textit{Flowers102}} & Zero-shot CLIP$_\text{ ICML'21}$\cite{radford2021clip} & \multicolumn{5}{c}{65.98}\\
\cline{2-7}
& CoOp$_\text{ IJCV'22}$\cite{Zhou2022coop} & $69.00 \pm 2.44$ & $78.47 \pm 1.88$  & $85.34 \pm 1.69$   &  $91.68 \pm 0.82$ & $94.47 \pm 0.36$ \\
& PLOT$_\text{ ICLR'23}$\cite{chen2023plot} & $71.09 \pm 1.44$ &  $81.22 \pm 0.92$ &  $87.61 \pm 0.79$  &  $92.60 \pm 0.55$ &  $\bm{95.18} \pm 0.40$  \\
& KgCoOp$_\text{ CVPR'23}$\cite{Yao2023kgcoop} & $68.73 \pm 1.97$ & $69.63 \pm 1.25$ &  $76.51 \pm 0.51$ & $80.71 \pm 0.63$ & $84.48 \pm 0.70$ \\
& ProGrad$_\text{ ICCV'23}$\cite{Zhu2023prograd} & $72.16 \pm 1.74$ & $79.55 \pm 0.88$ & $84.56 \pm 1.41$ & $91.73 \pm 0.35$ &  $94.10 \pm 0.41$\\
\cline{2-7}
%Tip-Adapter\cite{zhang2022tip} & $60.48\pm0.08$ & $60.56\pm0.16$ & $61.02\pm0.12$ & $61.24\pm0.08$ & $61.59\pm0.10$ \\
%\hline
& CLIP-Adapter$_\text{ IJCV'23}$\cite{Gao2023clipadapter} & $66.86 \pm 0.73 $ & $69.71 \pm 0.46$ & $77.42 \pm 0.60$ & $87.20 \pm 0.52$ & $ 91.16 \pm 0.23$ \\
& Tip-Adapter-F$_\text{ ECCV'22}$\cite{zhang2022tip} & $67.73 \pm 0.57$ & $68.18 \pm 0.84$ & $71.17 \pm 0.67$ & $84.11 \pm 0.49$ & $93.02 \pm 0.28$ \\
& Tip-Adapter-F*$_\text{ ECCV'22}$\cite{zhang2022tip} & $\bm{78.46} \pm 1.01$ & $\bm{85.14} \pm 0.81$ & $88.53 \pm 0.54$ & $92.33 \pm 0.32$ & $94.26 \pm 0.38$ \\
%\textcolor{blue}{(-0.48)}
\cline{2-7}
& Standard LP$_\text{ ICML'21}$\cite{radford2021clip} & $56.98 \pm 1.56$  &  $73.40 \pm 0.87$  &  $84.38 \pm 0.53$  &  $91.81 \pm 0.34$  & $95.05 \pm 0.29$  \\
& \cellcolor{blue!15}{LP++} & \cellcolor{blue!15}{$78.21 \pm 1.01$} & \cellcolor{blue!15}{$84.69 \pm 0.70$} & \cellcolor{blue!15}{$\bm{89.56} \pm 0.45$} & \cellcolor{blue!15}{$\bm{92.61} \pm 0.32$} & \cellcolor{blue!15}{$94.26 \pm 0.24$}\\
\midrule

\multirow{10}{*}{\textit{StanfordCars}} & Zero-shot CLIP$_\text{ ICML'21}$\cite{radford2021clip} & \multicolumn{5}{c}{55.78}\\
\cline{2-7}
& CoOp$_\text{ IJCV'22}$\cite{Zhou2022coop} & $57.00 \pm 0.93$& $58.96 \pm 0.78$ & $62.81 \pm 0.71$ & $68.40 \pm 0.61$ & $72.87 \pm 0.50$ \\
& PLOT$_\text{ ICLR'23}$\cite{chen2023plot} & $57.47 \pm 0.58$& $59.89 \pm 0.60$& $63.49 \pm 0.80$&  $68.75 \pm 0.46$ &  $73.86 \pm 0.39$  \\
& KgCoOp$_\text{ CVPR'23}$\cite{Yao2023kgcoop} & $57.19 \pm 0.65$  & $58.94 \pm 0.33$ & $59.85 \pm 0.51$ & $61.42 \pm 0.40$ & 
 $62.99 \pm 1.33$ \\
& ProGrad$_\text{ ICCV'23}$\cite{Zhu2023prograd} & $\bm{58.63} \pm 0.39$ & $\bm{61.23} \pm 0.65$ & $\bm{65.02} \pm 0.78$ & $\bm{69.43} \pm 0.40$ & $72.76 \pm 0.45$\\
\cline{2-7}
%Tip-Adapter\cite{zhang2022tip} & $60.48\pm0.08$ & $60.56\pm0.16$ & $61.02\pm0.12$ & $61.24\pm0.08$ & $61.59\pm0.10$ \\
%\hline
& CLIP-Adapter$_\text{ IJCV'23}$\cite{Gao2023clipadapter} & $56.67 \pm 0.22 $ & $57.94 \pm 0.27$ & $61.13 \pm 0.30$ & $65.43 \pm 0.10$ & $ 70.24 \pm 0.79$ \\
& Tip-Adapter-F$_\text{ ECCV'22}$\cite{zhang2022tip} & $57.24 \pm 0.23$ & $58.12 \pm 0.50$ & $59.34 \pm 0.20$ & $64.25 \pm 0.19$ & $71.38 \pm 0.23$  \\
& Tip-Adapter-F*$_\text{ ECCV'22}$\cite{zhang2022tip} & $57.85 \pm 0.33$ & $60.55 \pm 0.34$ & $64.22 \pm 0.52$ & $68.75 \pm 0.31$ & $\bm{74.19} \pm 0.30$ \\
%\textcolor{blue}{(-0.48)}
\cline{2-7}
& Standard LP$_\text{ ICML'21}$\cite{radford2021clip} & $22.94 \pm 0.61$  &  $35.48 \pm 0.51$  &  $47.49 \pm 0.67$  &  $59.34 \pm 0.30$  & $69.11 \pm 0.18$  \\
& \cellcolor{blue!15}{LP++} & \cellcolor{blue!15}{$57.20 \pm 0.65$} & \cellcolor{blue!15}{$59.95 \pm 0.36$} & \cellcolor{blue!15}{$63.44 \pm 0.34$} & \cellcolor{blue!15}{$67.81 \pm 0.24$} & \cellcolor{blue!15}{$72.33 \pm 0.18$}\\
\midrule
\end{tabular}
    \vspace{0.1cm}
    \caption{\textbf{Comparison to state-of-the-art methods.} Average classification accuracy (\%) and standard deviation over 10 tasks for 11 benchmarks, %averaged over the 11 classification benchmarks, 
    Best values are highlighted in bold.}
    \label{table:resultOther_AllDatasets_details}
\end{table*}

\begin{table*}[ht] 
\footnotesize
\tiny
\centering
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{l|lccccc}
\hline
 Dataset & \textbf{Number of shots ($S$)} & \textbf{1} & \textbf{2} & \textbf{4} & \textbf{8} & \textbf{16}\\
\hline
\hline
\multirow{10}{*}{\textit{FGVCAircraft}} & Zero-shot CLIP$_\text{ ICML'21}$\cite{radford2021clip} & \multicolumn{5}{c}{17.07}\\
\cline{2-7}
& CoOp$_\text{ IJCV'22}$\cite{Zhou2022coop} & $12.50 \pm 6.16$& $17.59 \pm 3.70$ & $21.27 \pm 2.54$& $26.85 \pm 0.63$& $31.20 \pm 0.40$ \\
& PLOT$_\text{ ICLR'23}$\cite{chen2023plot} & $17.75 \pm 1.36$ & $19.55 \pm 0.99$ & $22.26 \pm 0.89$& $26.70 \pm 0.70$  & $32.09 \pm 0.68$  \\
& KgCoOp$_\text{ CVPR'23}$\cite{Yao2023kgcoop} & $ 18.61 \pm 0.76$  &  $18.93 \pm 1.01$ & $21.16 \pm 0.82$ & $22.80 \pm 0.44$  & $24.10 \pm 0.59$ \\
& ProGrad$_\text{ ICCV'23}$\cite{Zhu2023prograd} & $18.41 \pm 0.98$  & $20.51 \pm 1.11$ & $23.65 \pm 0.50$ & $26.98 \pm 0.50$ & $30.47 \pm 0.76$\\
\cline{2-7}
%Tip-Adapter\cite{zhang2022tip} & $60.48\pm0.08$ & $60.56\pm0.16$ & $61.02\pm0.12$ & $61.24\pm0.08$ & $61.59\pm0.10$ \\
%\hline
& CLIP-Adapter$_\text{ IJCV'23}$\cite{Gao2023clipadapter} & $18.56 \pm 0.20 $ & $19.18 \pm 0.28$ & $21.00 \pm 0.21$ & $23.76 \pm 0.33$ & $ 33.37 \pm 0.23$ \\
& Tip-Adapter-F$_\text{ ECCV'22}$\cite{zhang2022tip} & $18.23 \pm 0.19$ & $19.12 \pm 0.20$ & $20.55 \pm 0.20$ & $23.60 \pm 0.29$ & $30.37 \pm 0.25$ \\
& Tip-Adapter-F*$_\text{ ECCV'22}$\cite{zhang2022tip} & $19.08 \pm 0.15$ & $20.79 \pm 0.59$ & $23.99 \pm 0.57$ & $\bm{30.58} \pm 0.29$ & $\bm{36.16} \pm 0.34$ \\
%\textcolor{blue}{(-0.48)}
\cline{2-7}
& Standard LP$_\text{ ICML'21}$\cite{radford2021clip} & $12.66 \pm 0.59$ &  $16.92 \pm 0.56$  &  $21.11 \pm 0.83$  &  $26.53 \pm 0.38$  &  $32.42 \pm 0.54$  \\
& \cellcolor{blue!15}{LP++} & \cellcolor{blue!15}{$\bm{19.69} \pm 0.39$} & \cellcolor{blue!15}{$\bm{21.58} \pm 0.46$} & \cellcolor{blue!15}{$\bm{24.22} \pm 0.60$} & \cellcolor{blue!15}{$27.73 \pm 0.48$} & \cellcolor{blue!15}{$31.73 \pm 0.44$}\\
\midrule
\multirow{10}{*}{\textit{EuroSAT}} & Zero-shot CLIP$_\text{ ICML'21}$\cite{radford2021clip} & \multicolumn{5}{c}{36.22}\\
\cline{2-7}
& CoOp$_\text{ IJCV'22}$\cite{Zhou2022coop} & $40.36 \pm 7.19$& $56.15 \pm 5.82$& $66.13 \pm 3.62$&  $77.02 \pm 1.78$ & $\bm{82.59} \pm 1.00$ \\
& PLOT$_\text{ ICLR'23}$\cite{chen2023plot} & $44.22 \pm 9.14$& $64.19 \pm 6.24$ & $69.37 \pm 3.26$&  $\bm{78.84} \pm 1.33$ & $81.76 \pm 1.43$  \\
& KgCoOp$_\text{ CVPR'23}$\cite{Yao2023kgcoop} & $43.86 \pm 9.17$  &  $ 52.92 \pm 5.92$  &  $ 59.51 \pm 3.46$  &  $63.23 \pm 3.03$   &  $64.04 \pm 1.40$ \\
& ProGrad$_\text{ ICCV'23}$\cite{Zhu2023prograd} & $49.37 \pm 5.03$ & $65.22 \pm 4.01$ & $69.57 \pm 2.88$  & $78.44 \pm 1.69$ & $82.17 \pm 0.98$\\
\cline{2-7}
%Tip-Adapter\cite{zhang2022tip} & $60.48\pm0.08$ & $60.56\pm0.16$ & $61.02\pm0.12$ & $61.24\pm0.08$ & $61.59\pm0.10$ \\
%\hline
& CLIP-Adapter$_\text{ IJCV'23}$\cite{Gao2023clipadapter} & $43.00 \pm 2.27 $ & $48.60 \pm 2.76$ & $59.15 \pm 2.26$ & $69.92 \pm 1.49$ & $ 75.38 \pm 0.78$ \\
& Tip-Adapter-F$_\text{ ECCV'22}$\cite{zhang2022tip} & $47.63 \pm 2.64$ & $57.62 \pm 1.86$ & $69.30 \pm 2.41$ & $75.22 \pm 1.32$ & $78.59 \pm 1.48$ \\
& Tip-Adapter-F*$_\text{ ECCV'22}$\cite{zhang2022tip} & $49.27 \pm 2.88$ & $\bm{65.66} \pm 1.39$ & $\bm{70.72} \pm 2.73$ & $74.66 \pm 3.15$ & $78.73 \pm 0.81$ \\
%\textcolor{blue}{(-0.48)}
\cline{2-7}
& Standard LP$_\text{ ICML'21}$\cite{radford2021clip} & $48.29 \pm 2.95$  & $56.81 \pm 2.93$   &  $64.99 \pm 3.47$  & $74.56 \pm 0.98$   &  $80.29 \pm 0.90$  \\
& \cellcolor{blue!15}{LP++} & \cellcolor{blue!15}{$\bm{57.23} \pm 1.63$} & \cellcolor{blue!15}{$61.65 \pm 1.66$} & \cellcolor{blue!15}{$68.67 \pm 2.21$} & \cellcolor{blue!15}{$75.86 \pm 0.99$} & \cellcolor{blue!15}{$80.53 \pm 1.05$}\\
\midrule

\multirow{10}{*}{\textit{OxfordPets}} & Zero-shot CLIP$_\text{ ICML'21}$\cite{radford2021clip} & \multicolumn{5}{c}{85.75}\\
\cline{2-7}
& CoOp$_\text{ IJCV'22}$\cite{Zhou2022coop} & $86.27 \pm 1.17$ &  $86.33 \pm 1.13$ & $85.34 \pm 1.69$   & $87.85 \pm 1.21$  & $88.68 \pm 0.71$ \\
& PLOT$_\text{ ICLR'23}$\cite{chen2023plot} & $87.15 \pm 0.72$ & $87.23 \pm 1.21$  &  $88.03 \pm 0.49$  & $88.38 \pm 0.64$  &  $88.23 \pm 0.54$  \\
& KgCoOp$_\text{ CVPR'23}$\cite{Yao2023kgcoop} & $87.51 \pm 0.68$  & $87.51 \pm 0.75$ & $88.04 \pm 0.46$ & $88.59 \pm 0.34$ &  $89.28 \pm 0.21$ \\
& ProGrad$_\text{ ICCV'23}$\cite{Zhu2023prograd} & $\bm{88.34} \pm 0.65$  & $\bm{87.88} \pm 0.69$ & $\bm{88.59} \pm 0.58$ & $\bm{88.87} \pm 0.42$ & $\bm{89.39} \pm 0.47$\\
\cline{2-7}
%Tip-Adapter\cite{zhang2022tip} & $60.48\pm0.08$ & $60.56\pm0.16$ & $61.02\pm0.12$ & $61.24\pm0.08$ & $61.59\pm0.10$ \\
%\hline
& CLIP-Adapter$_\text{ IJCV'23}$\cite{Gao2023clipadapter} & $85.46 \pm 0.48 $ & $86.37 \pm 0.25$ & $87.21 \pm 0.51$ & $87.95 \pm 0.26$ & $ 88.33 \pm 0.33$ \\
& Tip-Adapter-F$_\text{ ECCV'22}$\cite{zhang2022tip} & $85.70 \pm 0.16$ & $86.05 \pm 0.46$ & $86.40 \pm 0.29$ & $87.66 \pm 0.28$ & $89.08 \pm 0.27$ \\
& Tip-Adapter-F*$_\text{ ECCV'22}$\cite{zhang2022tip} & $86.05 \pm 0.36$ & $86.49 \pm 0.61$ & $87.19 \pm 0.36$ & $87.89 \pm 0.34$ & $88.26 \pm 0.37$ \\
%\textcolor{blue}{(-0.48)}
\cline{2-7}
& Standard LP$_\text{ ICML'21}$\cite{radford2021clip} & $30.62 \pm 1.61$  &  $42.64 \pm 2.03$  &  $55.60 \pm 0.98$  &  $67.32 \pm 0.98$  & $76.23 \pm 0.38$  \\
& \cellcolor{blue!15}{LP++} & \cellcolor{blue!15}{$84.24 \pm 1.36$} & \cellcolor{blue!15}{$85.74 \pm 0.56$} & \cellcolor{blue!15}{$86.94 \pm 0.48$} & \cellcolor{blue!15}{$87.71 \pm 0.65$} & \cellcolor{blue!15}{$88.38 \pm 0.61$}\\
\midrule

\multirow{10}{*}{\textit{Food101}} & Zero-shot CLIP$_\text{ ICML'21}$\cite{radford2021clip} & \multicolumn{5}{c}{77.35}\\
\cline{2-7}
& CoOp$_\text{ IJCV'22}$\cite{Zhou2022coop} & $75.58 \pm 1.29$  &  $77.49 \pm 0.41$ & $77.93 \pm 0.58$  &  $78.92 \pm 0.19$ & $79.21 \pm 0.36$ \\
& PLOT$_\text{ ICLR'23}$\cite{chen2023plot} & $77.46 \pm 0.55$ & $77.72 \pm 0.26$ & $78.23 \pm 0.25$ & $78.40 \pm 0.35$ & $78.86 \pm 0.19$  \\
& KgCoOp$_\text{ CVPR'23}$\cite{Yao2023kgcoop} & $77.20 \pm 0.77$  & $\bm{78.04} \pm 0.18$  & $77.97 \pm 0.28$ & $78.39 \pm 0.40$  &  $78.73 \pm 0.23$ \\
& ProGrad$_\text{ ICCV'23}$\cite{Zhu2023prograd} & $\bm{78.36} \pm 0.41$  & $78.01 \pm 0.70$ & $\bm{78.38} \pm 0.87$ & $\bm{79.11} \pm 0.18$ & $\bm{79.51} \pm 0.23$\\
\cline{2-7}
%Tip-Adapter\cite{zhang2022tip} & $60.48\pm0.08$ & $60.56\pm0.16$ & $61.02\pm0.12$ & $61.24\pm0.08$ & $61.59\pm0.10$ \\
%\hline
& CLIP-Adapter$_\text{ IJCV'23}$\cite{Gao2023clipadapter} & $76.93 \pm 0.19 $ & $77.22 \pm 0.15$ & $77.64 \pm 0.17$ & $77.97 \pm 0.22$ & $ 78.45 \pm 0.14$ \\
& Tip-Adapter-F$_\text{ ECCV'22}$\cite{zhang2022tip} & $77.53 \pm 0.14$  & $77.53 \pm 0.22$  & $77.82 \pm 0.27$ & $78.26 \pm 0.22$ & $78.99 \pm 0.15$ \\
& Tip-Adapter-F*$_\text{ ECCV'22}$\cite{zhang2022tip} & $77.58 \pm 0.10$ & $77.36 \pm0.39$ & $77.78 \pm0.15$ & $78.17\pm 0.11$ & $78.72\pm 0.06$ \\
%\textcolor{blue}{(-0.48)}
\cline{2-7}
&Standard LP$_\text{ ICML'21}$\cite{radford2021clip} & $31.59 \pm 1.20$  &  $44.60 \pm 1.03$  & $56.13 \pm 0.63$   &  $64.45 \pm 0.55$  &  $70.97 \pm 0.19$  \\
& \cellcolor{blue!15}{LP++} & \cellcolor{blue!15}{$76.61 \pm 0.77$} & \cellcolor{blue!15}{$77.22 \pm 0.55$} & \cellcolor{blue!15}{$77.79 \pm 0.34$} & \cellcolor{blue!15}{$78.53 \pm 0.14$} & \cellcolor{blue!15}{$78.88 \pm 0.19$}\\
\midrule

\end{tabular}
    \vspace{0.1cm}
    \caption*{Table ~\ref{table:resultOther_AllDatasets_details}. \textbf{Comparison to state-of-the-art methods} (Continued). Average classification accuracy (\%) and standard deviation over 10 tasks for 11 benchmarks, %averaged over the 11 classification benchmarks, 
    Best values are highlighted in bold.}
    
\end{table*}

\section{The implementation of L-BFGS optimizer}
When assessing the standard LP as in Table~\ref{table:resultOther_AllDatasets_details}, we follow the instructions provided in \cite{Zhou2022coop}, where the L-BFGS optimizer is implemented by NumPy, and used to optimize the standard CE loss jointly with L2 regularizers. As for the ablation study in Table~\ref{table:ablation-loss-and-optimizers}, all the optimizers are implemented by Pytorch, including L-BFGS\footnote{  \url{https://github.com/hjmshi/PyTorch-LBFGS}}. In this case, we did not use a regularizers for fair comparison.

==> sec/Rayleigh-and-minmax-theorem.tex <==
Let us first recall the well-known {\em Rayleigh quotient} the {\em min-max theorem}.

\paragraph{Rayleigh quotient} For a given symmetric  $D \times D$ real matrix $\bm{A}$, the Rayleigh quotient for $\bm{x} \in {\mathbb R}^D$ is 
given by:
\begin{equation}
R_{\bm{A}}(\bm{x}) = \frac{\bm{x}^t \bm{A} \bm{x}}{\|\bm{x}^2\|}
\end{equation}

\paragraph{Min-Max theorem}
Let $\lambda_{l}(\bm{A})$ denote the $l^\textrm{th}$ eigenvalue of $\bm{A}$, 
$\lambda_{max}(\bm{A}) = \max_{l} \sigma_{l}(\bm{A})$ and $\lambda_{min}(\bm{A}) = \min_{l} \sigma_{l}(\bm{A})$. 
The min–max theorem, also referred to as the variational principle, states that $R_{\bm{A}}$ is bounded above and below by 
$\lambda_{max}(\bm{A})$ and $\lambda_{min}(\bm{A})$:
\begin{equation}
\lambda_{min}(\bm{A}) \leq R_{\bm{A}}(\bm{x}) \leq  \lambda_{max}(\bm{A}) 
\end{equation}
Therefore, the largest and smallest eigenvalues of $\bm{A}$ admit the following variational characterization:
\begin{align}
\label{Rayleigh-optimization}
\lambda_{max}(\bm{A}) &= \max_{\bm{x}} R_{\bm{A}}(\bm{x}) \nonumber \\
\lambda_{min}(\bm{A}) &= \min_{\bm{x}} R_{\bm{A}}(\bm{x})
\end{align}
which is equivalent to the following quadratic-function optimization, s.t. unit-hyper-sphere constraint:
\begin{align}
\label{Quadratic-optimization}
\lambda_{max}(\bm{A}) &= \max_{\bm{x}} Q_{\bm{A}}(\bm{x}) \quad \mbox{s.t.} \quad \|\bm{x}\|=1  \nonumber \\
\lambda_{min}(\bm{A}) &= \min_{\bm{x}} Q_{\bm{A}}(\bm{x}) \quad \mbox{s.t.} \quad \|\bm{x}\|=1
\end{align}
where $Q_{\bm{A}}$ is the following quadratic function:
\begin{equation}
Q_{\bm{A}}(\bm{x}) = \bm{x}^t \bm{A} \bm{x} 
\end{equation}
This characterization enables to estimate the maximum and minimum eigen values with simple (efficient) iterative
procedures, e.g. the {\em power iteration}, also known as Von Mises iteration (more details on the procedure below).

\paragraph{Case 2: Lipschitz constants updated during iterations}

This starts to look like a real majorize-minimize! we also have two case, one if efficient and depends only on the class softmax predictions, the other is a bit less efficient and require computing the max eigenvalues iteratively (may not add much with the fast power iterations). \\ 

{\em Case 2.1: Efficient (closed-form) updates but looser)}

\begin{remark}
For unit-hypersphere feature embedding, i.e., $\|\bm{f}_i\| = 1$, we have:
\label{covariance-bound}
\begin{equation}
\label{covariance-bound-inequality}
    \lambda_{max}(\bm{A}_k) \leq \frac{1}{N}\sum_{i=1}^N (p_{ik} - p_{ik}^2)
\end{equation}
\end{remark}
This is due to:
\begin{align}
 \lambda_{max}(\bm{A}_k) &= \max_{\|\bm{x}\|=1} \bm{x}^t \left (\frac{1}{N}\sum_{i=1}^N (p_{ik} - p_{ik}^2) \bm{f}_i \bm{f}_i^t \right )  \bm{x} \nonumber \\
  & \leq  \frac{1}{N}\sum_{i=1}^N (p_{ik} - p_{ik}^2) \max_{\|\bm{x}\|=1} \bm{x}^t (\bm{f}_i \bm{f}_i^t) \bm{x} \nonumber \\
  & =  \frac{1}{N}\sum_{i=1}^N (p_{ik} - p_{ik}^2) \lambda_{max} (\bm{f}_i \bm{f}_i^t) \nonumber \\
  & =  \frac{1}{N}\sum_{i=1}^N (p_{ik} - p_{ik}^2) 
\end{align}
The last line is due to fact that $\lambda_{max} (\bm{f}_i \bm{f}_i^t) = 1$ when $\|\bm{f}_i\| = 1$. Indeed, it suffice to notice 
that $\bm{f}_i \bm{f}_i^t \bm{f}_i = \bm{f}_i \|\bm{f}_i\|^2 = \bm{f}_i$. This means $\bm{f}_i$ is an eigenvector and $1$ is the associated eigenvalue. Since $\lambda_{max} (\bm{f}_i \bm{f}_i^t) \leq \mbox{tr} (\bm{f}_i \bm{f}_i^t) = \|\bm{f}_i\|^2 = 1$, then $\lambda_{max} (\bm{f}_i \bm{f}_i^t) = 1$. 

The bound in \eqref{covariance-bound-inequality} suggests that we could update $1/\gamma_{\bm{w}}$ at each iteration in closed-form:
\begin{equation}
\label{update-gamma-closed-form}
\frac{1}{\gamma_{\bm{w}}} = \frac{N}{\sum_{i=1}^N (p_{ik} - p_{ik}^2)}
\end{equation}

{\em Case 2.2: Less efficient but more precise updates}

In fact, we can compute at each iteration an approximation of the maximum eigenvalue of $\bm{A}_k$ using the power iteration, which is given by the following iterations, starting from an initial value $\bm{x}^0$: 
\begin{equation}
\bm{x}^{l+1} = \frac{\bm{A}_k \bm{x}^{l}}{\|\bm{A}_k \bm{x}^{l}\|}  
\end{equation}
The most expensive computational part here is the matrix-vector multiplication $\bm{A}_k \bm{x}^{l}$. Also, a naive implementation that compute matrix $\bm{A}_k$ at each iteration will be inefficient (quadratic in $D$). However, in the particular case of matrices $\bm{A}$ taking the form $\bm{A} = \frac{1}{N}\sum_{i=1}^N \bm{f}_i \bm{f}_i^t$, we could have an efficient (linear complexity) implementation! {\bf Do not compute matrix $\bm{A}$ at each iteration, which will be quadratic in D}! Rather notice the following:
\begin{equation}
\left (\frac{1}{N}\sum_{i=1}^N \bm{f}_i \bm{f}_i^t \right ) \bm{x}^{l} =  
\sum_{i=1}^N  (\bm{f}_i^t \bm{x}^{l}) \bm{f}_i
\end{equation}
which is just a weighted mean feature vector: you compute the cosine similarities $(\bm{f}_i^t \bm{x}^{l})$ and then use them as weights in the sum. 
This has a complexity of $O(ND)$ whereas, in a naive implementation, just evaluating $A$ will have a complexity of $O(ND^2)$!

==> sec/method-maxime-paper.tex <==
\section{Robust MeanShift}
\paragraph{Mode finding MeanShift} We first introduce the MeanShift algorithm \cite{meanshift1975, mode_seeking1995, comaniciu1999mean, mean_shift_feature_analysis}, which will be later used in Section \ref{sec:ablation} as a specific case of our MTA. MeanShift is a procedure for locating the mode of a density function \cite{meanshift1975, mode_seeking1995} based on a kernel function, e.g. Gaussian kernel \cite{CarreiraPerpin2007GaussianMI}, by iteratively update an estimate towards denser regions. 
\begin{equation}
    \max_{m} \sum_{s \in S} K(x_s - m)
\end{equation}
which can be rewritten as a minimization problem. Alternatively, we can give a different weights for each point, which lead to a generalization of the common MeanShift algorithm \cite{mode_seeking1995}.
\begin{equation}
\label{eq:weighted_mean_shift}
    \min_{m} - \sum_{s \in S} K(x_s - m) w(s)
\end{equation}
\begin{prop}
\label{prop:cauchy}
Setting the gradients to 0 of Equation \ref{eq:weighted_mean_shift} with respect to m yields to a stationary point condition, for which we can find an unique solution via fixed-point iterations.
\begin{equation}
\label{eq:condition}
    m - g^i(m) = 0
\end{equation}
\begin{equation}
    \text{with } g^i(m) = \frac{\sum_{s \in S}  K(x_s - x) w(s) x_s}{\sum_{s \in S} K(x_s - x) w(s)}
\end{equation}
Then, 
\begin{equation}
m^{i,n+1} = g^{i}(m^{i,n})
\end{equation}
yield a Cauchy sequence $\{m^{i,n}\}_{n \in N}$. As such this sequence converges to a unique value $m_{i,*} = \lim_{n \xrightarrow{} \infty} m^{i,n}$. Furthermore, $m^{i,*}$ is the unique solution of the stationary-point condition in Equation \ref{eq:condition}.
\end{prop}
We summarize the MeanShift algorithm in Algorithm \ref{alg:meanshift}. Predicted class is computed by cosine similarity with the encoded prompts of each class k $t_k$, $\hat{k} = \argmax_{k} m^\intercal t_k$.

% Traditionnal mean shift ...
\begin{algorithm}
\caption{MeanShift \cite{meanshift1975}}\label{alg:meanshift}
\begin{algorithmic}
\Require bandwidth $b > 0$, tolerance threshold  $\epsilon > 0$, kernel K.
\State $m \gets x_0$
\While{$N \neq 0$}
\State $m(x) = \frac{\sum_{s \in S} K(x_s - x) x_s}{\sum_{s \in S} K(x_s - x)}$
\State $x \gets m(x)$
\EndWhile
\State $\hat{k} \gets \argmax_{k} m^\intercal t_k$
\end{algorithmic}
\end{algorithm}



% Introduction of Inlier-Outlier Score + explanation (see LAME and OSLO)
\paragraph{Robust MeanShift} 

\ismail{We give a first intuition on how robust MeanShift can behave when used with test-time augmentation as done in the next sections. Degenerated augmented views are unlikely to show similar and consistent features, creating either isolated data points or small regions with little structure. On the other hand, augmented views presenting major characteristics of the object to be recognized are likely to be projected close to the original image and close to each others. In this sense, inlierness score will spread to consistent augmented views and mode update will be attracted towards these regions.}

\ismail{Similarly to the test-time generalization setting recently introduced in \cite{}, assume that we are given a set of image samples $({\mathbf x}_p)_{1\leq p N}$, which correspond to $N$ distinct augmentations views of a given test sample ${\mathbf x}$. It is important to note that our method is applicable to any type of augmentations \cite{}, as shown in our experiments. Let ${\mathbf f}_p = \theta_v ({\mathbf x}_p)$ denote vision-encoded feature embedding corresponding to augmented sample ${\mathbf x}_p$, $\theta_v$ being the vision encoder of the CLIP pre-training model.} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% start formulation here - go back to pramble later %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this section, we introduce our formulation, which could be viewed as a novel extension of the popular mean-shift 
\cite{comaniciu1999mean}, an unsupervised procedure for finding the modes of the distribution of a given set 
of samples. In our case, we explicitly model and handle the potential presence of outliers in the estimation of the kernel density of the set of feature 
embeddings $({\mathbf f}_p)_{1 \leq p \leq N}$. To do so, we introduce a latent variable $y_p \in [0, 1]$ for each augmentation and propose to minimize the 
following robust mean-shift objective:
 
We find a latent assignment vector $\mathbf{y} = (y_p)_{1 \leq p \leq N} \in \Delta^{N-1}$, with 
$\Delta^{K-1} = \{{\mathbf y} \in [0, 1]^N \; | \; {\mathbf 1}^t {\mathbf y}   = 1 \}$ the probability simplex. 
\begin{align}
\label{eq:robust_mean_shift}
    \min_{{\mathbf m}, {\mathbf Y}} - \sum_{p=1}^N y_p K({\mathbf f}_p - {\mathbf m}) - \lambda \sum_{p, q} w_{p,q} y_p y_q  - \lambda_{\mathbf{y}} H({\mathbf y})
\end{align}
where the notations in problem (\ref{eq:robust_mean_shift}) are defined as follows: 
\begin{itemize}
\item {\bf Robust KDE}: Latent variable $y_p$ evaluates the \textit{inlierness} of the $p^{\mbox{{\small th}}}$ augmented view, 
i.e., the model's belief in ${\mathbf f}_p$ being an inlier or not within the whole set of augmented-view embeddings $({\mathbf f}_p)_{1 \leq p \leq N}$. Scores $y_p \in [0, 1]$ is high when the model considers the $p^{\mbox{{\small th}}}$ sample as an inlier, enabling it to contribute more in the KDE evaluation in (\ref{eq:robust_mean_shift}),  and small (closer to $0$) otherwise.    
\item {\bf Text-knowledge guided Laplacian regularization}: The pairwise affinities $w_{p,q}$ in the second term in (\ref{eq:robust_mean_shift}) are constructed form both the text and vision embeddings as follows. Let ${\mathbf s}_p \in \mathbb R^K$ denotes the text driven softmax prediction based on the zero-shot text embedding, i.e., the $k^{\mbox{{\small th}}}$ component of ${\mathbf s}_p$ is given by: 
%\begin{equation}
%s_{p,k} = \frac{\exp l_{p,k}} {\sum_{j=1}^K \exp l_{p,k}; \, l_{p,k} = \tau {\mathbf f}_p^t {\mathbf t}_k
%\end{equation}

\begin{equation}
w_{p,q} = \sigma (\tau {\mathbf f}_p)^t {\mathbf f}_p 
\end{equation}


\item $H({\mathbf y})$ is the Shannon entropy defined over simplex variables as follows: 
\begin{equation}
H({\mathbf y}) = - \sum_{p=1}^N y_p \ln y_p
\end{equation}
This term acts as a barrier function, forcing latent variable ${\mathbf y}$ to stay within the probability simplex.  

\item 
\end{itemize}







To take into account bad data augmentations, one may find useful to add an inlier/outlier score to the above objective function. We introduce a Laplacian regularizer \cite{JMLR:v7:belkin06a}, a common choice in graph clustering to encourage nearby points to have similar scores \cite{lame} and an entropic barrier to force our score to sum to 1. Leading to a concave-convex formulation that yields a parallel-structure algorithm with convergence guarantee.



We show that our Eq. \ref{eq:robust_mean_shift} can be minimized using the Concave-Convex Procedure \cite{cccp} to replace the concave parts of our minimization problem by their first-order approximation. This way, we derive an iterative bound optimization algorithm that computes independent updates of inlierness score variables $\xi$ at each iteration, and provably converges in Proposition \ref{prop:convergence}. Solving the Karush-Kuhn-Tucker (KKT) conditions yields to the following inlier/outlier update rule
\begin{align}
\label{eq:robust_inlier}
    \xi_s = \sigma \Big(\frac{1}{\lambda_{\xi}}(K(x_s - x) + \lambda \sum_{t \in S} w_{s,t} \xi_{t})\Big) \forall s \in S
\end{align}
We therefore have the new mode update, related to Equation \ref{eq:weighted_mean_shift}.
\begin{align}
\label{eq:robust_mode}
    m(x) = \frac{\sum_{s \in S} \xi_s K(x_s - x) x_s}{\sum_{s \in S} \xi_s K(x_s - x)}
\end{align} 

\begin{prop}
\label{prop:convergence} 
The sequence $\{\xi^{i}, m^{i}\}_{i \in N}$ from the alternate steps of ($\xi$-update) and (m-update) is converging and produce stationary points.
\end{prop}


\begin{algorithm}
\caption{Robust MeanShift (MTA)}\label{alg:robustmeanshift}
\begin{algorithmic}
\Require tolerance threshold  $\epsilon > 0$, kernel K.
\State $b \gets$ estimate\_bandwidth($x$)
\State $m \gets x_0$
\While{not converged}
    \While{not converged}
        \State Update $\xi$ according to (\ref{eq:robust_inlier})
    \EndWhile
    \While{not converged}
        \State Update m according to (\ref{eq:robust_mode})
    \EndWhile
\EndWhile
\State $\hat{k} \gets \argmax_{k} m^\intercal t_k$
\end{algorithmic}
\end{algorithm}
\paragraph{Interpretation}
Equation \ref{eq:robust_inlier} and \ref{eq:robust_mode} can be nicely interpreted on Figure \ref{fig:interpretation}. Subfigure \ref{fig:interpretation_inlier} shows how the inlierness scores are spreadind. A data point is given a high inlierness score if it is close to the mode and/or close to other data points with high inlierness scores. Therefore, inlierness score is spreading iteratively from data points close to the mode towards other data points controlled by their affinity relations. Subfigure \ref{fig:interpretation_mode} shows the update direction followed by traditional MeanShift (Algorithm \ref{alg:meanshift}) while the orange arrows follow the update of our Robust MeanShift (Algorithm \ref{alg:robustmeanshift}). Our mode update is directed towards dense regions with high inlierness scores, thus avoiding close regions with few or isolated data points.
\begin{figure}[t]
    \centering
    \begin{subfigure}{\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/inlier_interpretation.pdf} % Adjust width as needed
        \caption{\textbf{\textit{Inlierness score spread.}} Color gradation represents the inlierness score: the darker the higher.}
        \label{fig:interpretation_inlier}
    \end{subfigure}
    
    \begin{subfigure}{\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/mode_interpretation.pdf} % Adjust width as needed
        \caption{\textbf{\textit{Inlier density mode seeking.}} The white arrow represents the update diretion of the traditional MeanShift, instead our robust MeanShift follows the orange ones.}
        \label{fig:interpretation_mode}
    \end{subfigure}

    \caption{Interpretation of Equation \ref{eq:robust_inlier} (a) and Equation \ref{eq:robust_mode} (b). Our Robust MeanShift alternatively solves these 2 equations until convergence.}
    \label{fig:interpretation}
\end{figure}





